HyRRT-Connect: A Bidirectional Rapidly-Exploring Random Trees Motion Planning Algorithm for Hybrid Systems

This paper proposes a bidirectional rapidly-exploring random trees (RRT) algorithm to solve the motion planning problem for hybrid systems. The proposed algorithm, called HyRRT-Connect, propagates in both forward and backward directions in hybrid time until an overlap between the forward and backward propagation results is detected. Then, HyRRT-Connect constructs a motion plan through the reversal and concatenation of functions defined on hybrid time domains, ensuring the motion plan thoroughly satisfies the given hybrid dynamics. To address the potential discontinuity along the flow caused by tolerating some distance between the forward and backward partial motion plans, we reconstruct the backward partial motion plan by a forward-in-hybrid-time simulation from the final state of the forward partial motion plan. By applying the reversed input of the backward partial motion plan, the reconstruction process effectively eliminates the discontinuity and ensures that as the tolerance distance decreases to zero, the distance between the endpoint of the reconstructed motion plan and the final state set approaches zero. The proposed algorithm is applied to an actuated bouncing ball example and a walking robot example so as to highlight its generality and computational improvement.

==> macros/commands.tex <==
\newcommand{\pn}[1]{{\color{red} #1}}
\newcommand{\pnn}[1]{{\color{blue} #1}}
\newcommand{\pno}[1]{{\color{cyan} #1}}

\newcommand{\Reals}[1][]{\mathbb{R}^{#1}}
\newcommand{\Preals}[1][]{\mathbb{R}^{#1}_{\geq 0}}

\newbool{conf}
\setbool{conf}{false}

\ifbool{conf}{
% Items for conference version go in here.
}{
% Items for report version go in here.
 \addtolength{\oddsidemargin}{-.875in}
	\addtolength{\evensidemargin}{-.875in}
	\addtolength{\textwidth}{1.75in}
	\addtolength{\topmargin}{-.875in}
	\addtolength{\textheight}{1.75in} 
}

==> macros/packages.tex <==
\usepackage{./macros/hslTR}

\usepackage{graphics}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{verbatim}     
\usepackage{amsxtra}
\usepackage{epsfig}
\usepackage{subfigure}
\usepackage{hyperref} 
\usepackage{amsmath}
\usepackage{latexsym}
\usepackage{ifthen}
\usepackage{psfrag}
\usepackage{subfigure}
\usepackage{color}
\usepackage{float}
\usepackage{tikz}
\usepackage{mathtools}
\usepackage{etoolbox}
\usepackage{enumitem}

\usepackage{./macros/rgsEnvironments}
\usepackage{./macros/rgsMacros}  

\usepackage{algorithm}
\usepackage{algpseudocode}

\usetikzlibrary{shapes,arrows}

==> macros/theorems.tex <==
 \newcounter{theorem}
\newtheorem{problem}[theorem]{Problem}

\newcommand{\incfig}[2][1]{%
	\def\svgwidth{#1\columnwidth}
	\import{./figures/}{#2.pdf_tex}
}

\DeclareMathOperator{\interior}{int}
\DeclareMathOperator*{\argmin}{arg\,min}

\newlist{steps}{enumerate}{1}
\setlist[steps, 1]{leftmargin=45pt, label = \textbf{Step \arabic*}:}

==> sections/BiHyRRT/searchtree.tex <==
Each search tree is modeled by a directed tree. A directed tree $\mathcal{T}$ is a pair $\mathcal{T} = (V, E)$, where $V$ is a set whose elements are called vertices and $E$ is a set of paired vertices whose elements are called edges. The edges in the directed tree are directed, which means the pairs of vertices that represent edges are ordered. The set of edges $E$ is defined as
$
E \subseteq \{(v_{1}, v_{2}): v_{1}\in V, v_{2}\in V, v_{1}\neq v_{2}\}.
$
The edge $e = (v_{1}, v_{2})\in E$ represents an edge from $v_{1}$ to $v_{2}$.  
A path in $\mathcal{T} = (V, E)$ is a sequence of vertices
$
p = (v_{1}, v_{2}, ..., v_{k})
$ such that $(v_{i}, v_{i + 1})\in E$ for all $i= 1, 2,..., k - 1$.
HyRRT-Connect constructs a forward-in-time search tree, denoted $\fw{\stree} = (\fw{V}, \fw{E})$ and a backward-in-time search tree, denoted $\bw{\stree} = (\bw{V}, \bw{E})$. Each vertex in the search tree $\fw{\stree}$ (respectively, $\bw{\stree}$) is associated with a state value of $\hs$ (respectively, $\bw{\hs}$). Each edge in $\fw{E}$ (respectively, $\bw{E}$) is associated with a solution pair to $\hs$ (respectively, $\bw{\hs}$) that connects the state values associated with their endpoint vertices. The state value associated with vertex $v\in \fw{V}\cup \bw{V}$ is denoted as $\overline{x}_{v}$ and the solution pair associated with edge $e\in \fw{E}\cup \bw{E}$ is denoted as $\overline{\psi}_{e}$.

The solution pair that the path $p = (v_{1}, v_{2}, ..., v_{k})$ represents is the concatenation of all the solutions associated with the edges therein, namely,
\begin{equation}
\label{equation:concatenationpath}
\tilde{\psi}_{p} := \overline{\psi}_{(v_{1}, v_{2})}|\overline{\psi}_{(v_{2}, v_{3})}|\ ...\  |\overline{\psi}_{(v_{k-1}, v_{k})}	
\end{equation}
where $\tilde{\psi}_{p}$ denotes the solution pair associated with the path $p$. For the notion of concatenation, see Definition \ref{definition:concatenation}. 
%An example of the path $p$ and its associated solution pair $\tilde{\psi}_{p}$ is shown in Figure \ref{fig:searchgraph}.

The proposed Bi-HyRRT-Connect algorithm requires a library of possible inputs to construct $\fw{\stree}$, denoted $\fw{\il} = (\fw{\il}_{C}, \fw{\il}_{D})$, and a library of possible inputs to construct $\bw{\stree}$, denoted $\bw{\il} = (\bw{\il}_{C}, \bw{\il}_{D})$. The input library $\fw{\il}$ (respectively, $\bw{\il}$) includes the input signals that can be applied during flows, collected in $\fw{\il}_{C}$ (respectively, $\bw{\il}_{C}$), and the input values that can be applied at jumps, collected in $\fw{\il}_{D}$ (respectively, $\bw{\il}_{D}$).

==> sections/backwardsystem/backwardhybridsystem.tex <==
In the proposed template, a backward-in-time version of the hybrid system $\mathcal{H} = (C, f, D, g)$, denoted $\mathcal{H}^{\text{bw}} = (C^{\text{bw}}, f^{\text{bw}}, D^{\text{bw}}, g^{\text{bw}})$, is required when propagating trajectories backward in hybrid time. The backward-in-time hybrid system $\mathcal{H}^{\text{bw}}$ is constructed as follows.
\begin{definition}
	(Backward-in-time hybrid system) Given a hybrid system $\mathcal{H} = (C, f, D, g)$, the backward-in-time hybrid system of $\mathcal{H}$, denoted $\mathcal{H}^{\text{bw}}$, is the hybrid system
	\begin{equation}
	\mathcal{H}: \left\{              
	\begin{aligned}               
	\dot{x} & =  f^{\text{bw}}(x, u)     &(x, u)\in C^{\text{bw}}\\                
	x^{+} & \in  g^{\text{bw}}(x, u)      &(x, u)\in D^{\text{bw}}\\                
	\end{aligned}   \right. 
	\label{model:generalhybridbackwardsystem}
	\end{equation}
	where
	\begin{enumerate}[label = \arabic*)]
		\item The backward-in-time flow set is constructed as
		\begin{equation}
		\label{equation:backwardflowset}
		C^{\text{bw}} := C.
		\end{equation}
		\item The backward-in-time flow map is constructed as
		\begin{equation}
		\label{equation:backwardflow}
		\begin{aligned}
		f^{\text{bw}}(x, u) :=  -f(x, u) \quad \forall (x, u)\in C^{\text{bw}}.
		\end{aligned}
		\end{equation} 
		\item The backward-in-time jump map is constructed as
		\begin{equation}
		\label{set:gbw}
		\begin{aligned}
		g^{\text{bw}}(x, u) := \{z\in \mathbb{R}^{n}:\  x = g(z, u), (z, u)\in D\} \quad \forall (x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}.
		\end{aligned}
		\end{equation}
		\item The backward-in-time jump set is constructed as
		\begin{equation}
		\label{set:dbw}
		\begin{aligned}
		D^{\text{bw}} := \{(x, u)\in \mathbb{R}^{n}\times \mathbb{R}^{m}: \exists z\in g^{\text{bw}} (x, u): 
		(z, u)\in D\}.
		\end{aligned}
		\end{equation}
	\end{enumerate}
\end{definition}
The above shows a general method of constructing the backward-in-time system given the forward-in-time hybrid system. Note that although the jump map $g$ in the forward-in-time system $\mathcal{H}$  is a single-valued map, the jump map $g^{\text{bw}}$ in the backward-in-time system $\mathcal{H^{\text{bw}}}$ is not necessarily single valued. Hence, a difference inclusion is used in (\ref{model:generalhybridbackwardsystem}). 
\begin{example}\label{example:bouncingballbw}
	(Actuated bouncing ball system in Example \ref{example:bouncingball}, revisited) The backward-in-time hybrid system of the actuated bouncing ball system is constructed as follows.
	\begin{itemize}
		\item From (\ref{equation:backwardflowset}), the backward-in-time flow set $C^{\text{bw}}$ is given by
		\begin{equation}
		\label{equation:bouncingballbwflowset}
		C^{\text{bw}} := C =  \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1} \geq 0\}.
		\end{equation}
		\item From (\ref{equation:backwardflow}), the backward-in-time flow map $f^{\text{bw}}$ is given by
		\begin{equation}
		\label{equation:bouncingballbwflowmap}
		f^{\text{bw}}(x, u) := -f(x, u) = \left[ \begin{matrix}
		-x_{2} \\
		\gamma
		\end{matrix}\right] \qquad (x, u)\in C^{\text{bw}}.
		\end{equation}
		\item From (\ref{set:dbw}), the backward-in-time jump set is given by
		\begin{equation}
		\label{equation:bouncingballbwjumpset}
		D^{\text{bw}} := \{(x, u)\in \mathbb{R}^{2}\times \mathbb{R}: x_{1} = 0, x_{2} \geq u, u\geq 0\}. 
		\end{equation}
		\item From (\ref{set:gbw}), the backward-in-time jump map $g^{\text{bw}}$ is given by 
		\begin{equation}
		\label{equation:bouncingballbwjumpmap}
		g^{\text{bw}}(x, u) :=  \left[ \begin{matrix}
		x_{1} \\
		-\frac{x_{2}}{\lambda}+\frac{u}{\lambda}
		\end{matrix}\right] \qquad (x, u)\in D^{\text{bw}}.
		\end{equation}
	\end{itemize}
	%	In conclusion, the backward-in-time hybrid system is given by:
	%	\begin{equation}
	%	\cal{H}^{\text{bw}}: \left\{              
	%	\begin{aligned}               
	%	\dot{x} &= f^{\text{bw}}(x, u)    &(x, u)\in C^{\text{bw}}\\                
	%	x^{+} &=  g^{\text{bw}}(x, u)    &(x, u)\in D^{\text{bw}}\\                
	%	\end{aligned}   \right.   
	%	\label{model:bouncingballbw}
	%	\end{equation}
	%	where the flow map $f$ is given in (\ref{equation:bouncingballbwflowmap}), the flow set $C$ is given in (\ref{equation:bouncingballbwflowset}), the jump map $g$ is given in (\ref{equation:bouncingballbwjumpmap}) and the jump set $D$ is given in (\ref{equation:bouncingballbwjumpset}).
\end{example}
 Proposition \ref{theorem:reversedarcbwsystem} shows that the reversal of the solution pair to a hybrid system is a solution pair to its backward-in-time hybrid system.
\begin{proposition}
	\label{theorem:reversedarcbwsystem}
	Given a hybrid system $\mathcal{H}$ and its backward-in-time system $\mathcal{H^{\text{bw}}}$, if $\psi = (\phi, u)$ is a compact solution pair to $\mathcal{H}$, the reversal $\psi' = (\phi', u')$ of $\psi = (\phi, u)$ is a compact solution pair to $\mathcal{H}^{\text{bw}}$.
\end{proposition}
\begin{proof}
	To be completed...
\end{proof}
